Trackers Bounce Back: Measuring Evasion of Partitioned Storage in the Wild

This work presents a systematic study of navigational tracking, the latest development in the cat-and-mouse game between browsers and online trackers. Navigational tracking allows trackers to 'aggregate users' activities and behaviors across sites by modifying their navigation requests. This technique is particularly important because it circumvents the increasing efforts by browsers to partition or block third-party storage, which was previously necessary for most cross-website tracking. While previous work has studied specific navigational tracking techniques (i.e. "bounce tracking"), our work is the first effort to systematically study and measure the entire category of navigational tracking techniques. We describe and measure the frequency of two different navigational tracking techniques on the Web, and find that navigational tracking is present on slightly more than ten percent of all navigations that we made. Our contributions include identifying 214 domains belonging to at least 104 organizations tracking users across sites through link decoration techniques using direct or indirect navigation flows. We identify a further 23 domains belonging to at least 16 organizations tracking users through bounce tracking (i.e. bouncing users through unrelated third parties to generate user profiles). We also improve on prior techniques for differenting user identifiers from non-sensitive information, which is necessary to detect one class of navigational tracking. We discuss how our findings can used to protect users from navigational tracking, and commit to releasing both our complete dataset and our measurement pipeline

==> introduction.tex <==
\section{Introduction}

\begin{itemize}
\item Users have become increasingly concerned about web trackers
\item Tracking a user across websites is more concerning than tracking a user 
within a single website~\cite{citation_needed}
\item Accordingly, browsers have started to block third-party cookies by 
default 
(Safari~\cite{itp}, Brave\cite{brave_antibounce}) or provide 
an option to do so (Firefox\cite{etp}). Chrome is planning to 
offer this functionality in the 
future~\cite{privacy_sandbox_milestones}. 
\item \emph{Pivot}: Trackers are looking for ways to avoid  
the new protections~\cite{szikszai_future_proof, 
rakuten_navigating_2020, rakuten_overcoming_2021, 
tune_server_side,digiday_s2s,tinuiti_s2s,twilio_segment_s2s, 
awin_itp_reaction_2020, 
szikszai_responded_itp_2018, cj_itp_part2}. Describe 
bounce 
tracking~\cite{baycloud_criteo_2015, 
brave_redirection_2018}.
\item We make the following contributions:
	\begin{itemize}
		\item We generalize tracking behavior beyond bounce tracking to any 
		information sharing that would circumvent partitioned storage, 
		including link decoration. We refer to such illicit information transfers as ``token 
		smuggling''/``navigational tracking.'' (pick one)
		\item We measure the prevalence of such information sharing in the wild 
		using random walks of the web starting at the Alexa Top 15k.
		\item We present a categorization of trackers' behaviors, including which categories of sites 
		are more likely to engage in token smuggling, and how tokens are commonly transferred. 
		\item We present countermeasures against information sharing?
	\end{itemize}

\end{itemize}

Note: We aren't interested it sites recording that an anonymous user 
came from some previous site. We specifically want to know when sites 
are passing \emph{user identifiers} between sites: when they know not 
only where you came from and who they think you are, but who the 
other site thinks you are.

Say something about how cookie syncing is not what we're looking for: we're 
looking for a tracker 
tracking a user across multiple websites, not trackers sharing identifiers on a 
single website. Cookie 
syncing is mentioned by at least A Calculus of Tracking: Theory and Practice, 
WEBGRAPH: Capturing 
Advertising and Tracking Information Flows for Robust Blocking, and 
\cite{fouad2018missed}.


